Partial Optimality in Cubic Correlation Clustering

The higher-order correlation clustering problem is an expressive model, and recently, local search heuristics have been proposed for several applications. Certifying optimality, however, is NP-hard and practically hampered already by the complexity of the problem statement. Here, we focus on establishing partial optimality conditions for the special case of complete graphs and cubic objective functions. In addition, we define and implement algorithms for testing these conditions and examine their effect numerically, on two datasets.

==> section-multicut.tex <==
\section{Connection to the Cubic Multicut Problem}\label{sec: multicut}

In this section, we turn to a natural question that arises in the context of correlation clustering and multicuts.
When the objective functions are linear, it is well-known that the two problems are equivalent. \note{cite!}
In particular, the feasible vectors of the two problems are in a 1-to-1 correspondence given by the affine map $x \mapsto 1 - x$.
This implies that the optimal value of the (linear) correlation clustering problem is equal to a constant minus the optimal value of the (linear) multicut problem. 
It is therefore reasonable to ask ourselves whether the same behaviour occurs also in the nonlinear setting. 
One important thing to realize is that, while the cubic term in \eqref{eq: pb} tells us exactly what we want, i.e., it is equal to one if and only if all the three corresponding points are in the same cluster, this expressiveness property does not transfer to the higher-order multicut problem.
OIn fact, if we simply replace the variables with their affine transformation $x \mapsto 1 - x$, the cubic term becomes $(1 - x_{pq})(1 - x_{pr})(1 - x_{qr})$ for $pqr \in \binom S3$. 
We observe that this product equals one if and only if all the correlation clustering variables $x_{pq}$, $x_{pr}$, $x_{qr}$ have value zero, meaning that the three points end up in three different clusters. 
However, we would desire the cubic term in the multicut problem to evaluate $1$ also when two points out of three are together but the third one is in another cluster. 
This suggests that the higher-order multicut problem cannot be expressed naturally without the introduction of additional variables, contrary to the higher-order correlation clustering problem. 
Next, we define the variables of the cubic multicut problem, and show the relationship between the optimal values of this problem and of the cubic correlation clustering. 

\begin{gather}
\forall pq \in \binom S2, \qquad z_{pq} := 1 - x_{pq} = \begin{cases}
1, \qquad & \text{if } $p, q$ \text{ are in different clusters,} \\
0, \qquad & \text{if } $p, q$ \text{ otherwise}, 
\end{cases} \\
\forall pqr \in \binom S3, \qquad y_{pq} := 1 - x_{pq}x_{pr}x_{qr} = \begin{cases}
1, \qquad & \text{if } $p, q, r$ \text{ are not all together,} \\
0, \qquad & \text{if } $p, q, r$ \text{ otherwise}.
\end{cases}
\end{gather}

Then, the cubic multicut problem with respect to costs $c \in \mathbb{R}^{\binom S3 + \binom S2 + 1}$ is: \note{constraints?}
\begin{align}
\min \quad & \sum_{pqr \in \binom S3} c_{pqr} y_{pqr} + \sum_{pq \in \binom S2} c_{pq} z_{pq} + c_{\emptyset} \\
\text{s.t. } & XXX \ .
\end{align}

Regarding the objective values:
\begin{align}
\text{obj}_{\text{CCC}} & = \sum_{pqr \in \binom S3} c_{pqr} x_{pq}x_{pr}x_{qr} + \sum_{pq \in \binom S2} c_{pq} x_{pq} + c_{\emptyset} \\ 
& = \sum_{pqr \in \binom S3} c_{pqr} - \sum_{pqr \in \binom S3} c_{pqr} (1 - x_{pq}x_{pr}x_{qr}) + \sum_{pq \in \binom S2} c_{pq} - \sum_{pq \in \binom S2} c_{pq} (1 - x_{pq}) - c_{\emptyset} + 2c_{\emptyset} \\
& = - \text{obj}_\text{CMC} + C, 
\end{align}
where $C$ is a constant (specifically, $C = \sum_{pqr \in \binom S3} c_{pqr} + \sum_{pq \in \binom S2} c_{pq} + 2c_{\emptyset}$).

We conclude that the two problems are equivalent similarly to the linear case, even if here the two problems have a different number of variables.
Hence, all partial optimality results obtained for one problem can be transferred to the other problem once we flip the sign of the costs and the binary values of the variables.


